A short proof that ${\mathcal B}(L_1)$ is not amenable

Non-amenability of ${\mathcal B}(E)$ has been surprisingly difficult to prove for the classical Banach spaces, but is now known for $E= \ell_p$ and $E=L_p$ for all $1\leq p<\infty$. However, the arguments are rather indirect: the proof for $L_1$ goes via non-amenability of $\ell^\infty({\mathcal K}(\ell_1))$ and a transference principle developed by Daws and Runde (Studia Math., 2010). In this note, we provide a short proof that ${\mathcal B}(L_1)$ and some of its subalgebras are non-amenable, which completely bypasses all of this machinery. Our approach is based on classical properties of the ideal of representable operators on $L_1$, and shows that ${\mathcal B}(L_1)$ is not even approximately amenable.

==> BL1namac.tex <==

\usepackage{amsmath,amsfonts,amssymb}

\numberwithin{equation}{section}

% YC FORCE OF HABIT
\newcommand{\defeq}{\mathbin{:=}}
\newcommand{\dt}[1]{{\sf {#1}}}
\newcommand{\iso}{\cong}
\newcommand{\fu}[1]{{#1}^{\sharp}}    % forced unitisation
\newcommand{\Nat}{{\mathbb N}}
\newcommand{\Cplx}{{\mathbb C}}
\newcommand{\Bdd}{{\mathcal B}}
\newcommand{\Om}{\Omega}
\newcommand{\veps}{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bbA}{{\mathbb A}}

\newcommand{\fR}{{\mathfrak R}}
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cW}{{\mathcal W}}


\newcommand{\norm}[1]{{\Vert#1\Vert}}
\newcommand{\ptp}{\mathbin{\widehat{\otimes}}} % projective tensor product
\newcommand{\tp}{\mathbin{\otimes}} % projective tensor product

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% THEOREMS ETC


\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


%Styles for theorems, definitions, remarks

\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem*{thmstar}{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem*{notn}{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}

